Structured Inference Networks for Nonlinear State Space Models

Gaussian state space models have been used for decades as generative models of sequential data. They admit an intuitive probabilistic interpretation, have a simple functional form, and enjoy widespread adoption. We introduce a unified algorithm to efficiently learn a broad class of linear and non-linear state space models, including variants where the emission and transition distributions are modeled by deep neural networks. Our learning algorithm simultaneously learns a compiled inference network and the generative model, leveraging a structured variational approximation parameterized by recurrent neural networks to mimic the posterior distribution. We apply the learning algorithm to both synthetic and real-world datasets, demonstrating its scalability and versatility. We find that using the structured approximation to the posterior results in models with significantly higher held-out likelihood.

==> model_config.tex <==
\section{Model Configurations}
We detail the model configurations used in the experimental section. 

In each instance, we detail the model architecture used in the generative model (comprising a transition and emission function)
as well as the model used for posterior inference. 

``L'' denotes a linear layer with the values in parenthesis denoting the dimensions of the transformation. ``NL'' denotes the application
of a non-linearity (specified in the caption). 
Since parameters in the model are shared across time, 
we describe the architecture at a single time-step. 
The row denoted ``Inference'' is the architecture used for performing inference. 
In the case of the bidirectional RNN, we concatenate the outputs
from the forward and reverse RNN to perform prediction of the posterior means and log covariances. 
The recognition network predicts the posterior mean and log-covariance. 
The two quantities are predicted with a shared base network feeding into a separate final linear layer (i.e the last linear layer in the row 
``Inference'' is different for the function used to predict the posterior mean and the posterior log-covariance). Square braces indicate a vector concatenation
operation.

Table \ref{tab:model_synthetic} describes the model architecture used in the synthetic experiments. We detail the architectures used for inference in 
``MF-LR'' and ``ST-LR''. The other inference algorithms involve different structures in the LSTM-RNN module but are otherwise identical. The ``combiner function'' is 
detailed by the mapping from $[h_t;z_{t-1}]$\rarr$\mu_q$.

Table \ref{tab:model_polyphonic} describes the architecture used for the polyphonic dataset
and in Table \ref{tab:model_medical}, we describe the architecture used for experiments on medical data. 

\begin{table}[h]
\centering
\caption{Synthetic Experiments (ReLU was used as the non-linearity)}
\label{tab:model_synthetic}
\begin{tabular}{@{}ccc@{}}
\toprule
Inference (MF-LR) & $x_t$ \rarr \LNL{1}{20}\rarr \LNL{20}{20} \rarr \LNL{20}{20} \rarr \bLSTM{2}{20}{20} \\& \rarr \LNL{40}{20} \rarr \LNL{20}{20} \rarr \Lin{20}{1} \rarr $\mu_q$ or $\log\sigma_q^2$\\ \midrule
Inference (ST-LR) & $x_t$ \rarr \LNL{1}{20}\rarr \LNL{20}{20} \rarr \LNL{20}{20} \rarr \bLSTM{2}{20}{20} \\& \rarr \LNL{40}{20} \rarr $h_t$\\&
			$[h_t;z_{t-1}]$ \rarr \LNL{20+1}{20} \rarr \LNL{20}{20}\rarr\Lin{20}{1} \rarr $\mu_q$ or $\log\sigma_q^2$\\ \midrule
Emission   &  Fixed\\ \midrule
Transition &  Fixed\\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Polyphonic Experiments (Tanh was used as the non-linearity).}
\label{tab:model_polyphonic}
\begin{tabular}{@{}ccc@{}}
\toprule
Inference  & $x_t$ \rarr \LNL{88}{200}\rarr \LNL{200}{200} \rarr \LNL{200}{200} \rarr \LSTM{2}{200}{200}\\& \rarr \Lin{200}{200} \rarr $\mu_q$ or $\log\sigma_q^2$\\ \midrule
Emission   & Z\rarr \LNL{200}{200} \rarr \LNL{200}{200} \rarr \LNL{200}{200} \rarr \Lin{200}{200} \rarr Sigmoid \\\midrule
Transition ($\mu_p$) & Z\rarr \LNL{200}{200} \rarr \LNL{200}{200} \rarr \Lin{200}{200} \\\midrule
Transition ($\log\sigma_p^2$)& Z\rarr \LNL{200}{200} \rarr \LNL{200}{200} \rarr \Lin{200}{200} \\\midrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Medical Experiments (Tanh was used as the non-linearity). We describe the ``E:NL-T:NL'' model. The observations were $48$ dimensional of which there were $4$ lab indicators that we treat separately to perform
do-calculus.}
\label{tab:model_medical}
\begin{tabular}{@{}ccc@{}}
\toprule
Inference  & $[x_t; u_{t}]$ \rarr \LNL{48+8}{200}\rarr \LNL{200}{300} \rarr \LNL{200}{200}\\& \rarr \bLSTM{2}{200}{200} \rarr \Lin{400}{20} \rarr $\mu_q$ or $\log\sigma_q^2$\\ \midrule
Emission (Lab Indicators $i_t$ )  & $z_t$ \rarr \LNL{20}{200} \rarr \Lin{200}{4} \rarr Sigmoid \\\midrule
Emission (Lab Values \& Diagnosis Codes) & $[z_t; i_t]$ \rarr \LNL{20+4}{200} \rarr \Lin{200}{44} \rarr Sigmoid \\\midrule
Transition ($\mu_p$) & $[z_t;u_t]$ \rarr \LNL{20+8}{200} \rarr \LNL{200}{200} \rarr \Lin{200}{20} \\\midrule
Transition ($\log\sigma_p^2$)& Fixed with dimension $20$ (Sampled from Uniform(-1,1)\\ \bottomrule 
\end{tabular}
\end{table}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

